Dynamic Matching with Post-allocation Service and its Application to Refugee Resettlement

Motivated by our collaboration with a major refugee resettlement agency in the U.S., we study a dynamic matching problem where each new arrival (a refugee case) must be matched immediately and irrevocably to one of the static resources (a location with a fixed annual quota). In addition to consuming the static resource, each case requires post-allocation services from a server, such as a translator. Given the uncertainty in service time, a server may not be available at a given time, thus we refer to it as a dynamic resource. Upon matching, the case will wait to avail service in a first-come-first-serve manner. Bursty matching to a location may result in undesirable congestion at its corresponding server. Consequently, the central planner (the agency) faces a dynamic matching problem with an objective that combines the matching reward (captured by pair-specific employment outcomes) with the cost for congestion for dynamic resources and over-allocation for the static ones. Motivated by the observed fluctuations in the composition of refugee pools across the years, we aim to design algorithms that do not rely on distributional knowledge. We develop learning-based algorithms that are asymptotically optimal in certain regimes, easy to interpret, and computationally fast. Our design is based on learning the dual variables of the underlying optimization problem; however, the main challenge lies in the time-varying nature of the dual variables associated with dynamic resources. Our theoretical development brings together techniques from Lyapunov analysis, adversarial online learning, and stochastic optimization. On the application side, when tested on real data from our partner agency and incorporating practical considerations, our method outperforms existing ones making it a viable candidate for replacing the current practice upon experimentation.

==> tex/main/EC+lit+review+main.tex <==
% lit review for EC version 
% EC version
\subsection{Further Related Work}\label{subsec:lit+review}

\SLcomment{EC Flagging: significantly shortend, and other parts moved to appendix}
\SLcomment{Flagging for myself; make sure to reflect this in the intro}

Our work relates and contributes to the literature on refugee matching systems, online resource allocation, and control of queueing systems. In the following, due to space limitation, we only highlight the most closely related work and kindly refer readers to \SLedit{Appendix \ref{apx+EC+lit+review}} for more extensive literature review. 
% applilcation side
On the application side, the work of \citet{bansak2022outcome} is the most proper point of comparison as they also consider an objective that penalizes congestion. However, tied cases are not modeled and thus the over-allocation cost is not included in the objective. We modify their proposed sampling-based \SLedit{heuristics} to incorporate tied cases and then compare its performance to that of our method. As we show in  \Cref{sec:numerics}, when tested on real data, our method performs substantially better thanks to its robustness. \VMedit{Further, unlike previous work including \citet{bansak2022outcome}, we take a theoretical approach with provable performance guarantees}. 

From a methodological standpoint, closest to our work is that of \citet{agrawal2014dynamic} and \citet{balseiro2021regularized}. These studies consider online resource allocation with an assumption that a (non-linear) convex objective can only depend on {\em total} allocation of resources. Due to this assumption, the offline problem has only a few time-invariant dual variables which can then be learned fast enough to ensure low regret. We leverage similar ideas to the aforementioned papers to learn dual variables corresponding to static resources. However, such assumption {\em fails} for the average backlogs in our objective because the associated dual variables are time-varying and thus cannot be learned using similar ideas. This subtle difference led us to go well beyond the machinery of the aforementioned papers and to bring new tools from drift analysis and stochastic first-order methods (notably their high probability last-iterate convergence property) to design and analyze low-regret algorithms. In a similar vein, we also highlight that our objective function does not satisfy the ``exchangeability'' condition imposed in the recent work of \citet{freund2019good} due to the inherent dynamic nature of the backlogs (see \Cref{apx+EC+lit+review} for more discussions).




==> tex/main/Full+lit+review.tex <==
\subsection{Related Literature}\label{subsec:lit+review}
Our work relates and contributes to several streams of literature.\par 
{\bf Matching Policies for Refugee Resettlement:} 
{There has been growing academic interest in designing matching policies for refugee resettlement, leading to the two main approaches. The first approach is to consider a centralized \emph{outcome-based} system, focusing on integration outcomes such as employment within 90 days, and design matching algorithms that target such objectives. Central to the outcome-based approach is the development of ML models that predict employment outcomes for a pair of case and affiliate~ \citep{bansak2018improving, bansak2024learning}. Equipped with such models, several recent papers, including ours, aim to optimize matching decisions to improve employment, taking into account some of the operational considerations  discussed in or fairness criteria \Cref{subsec:intro+background} \citep{golz2019migration, ahani2021placement,
ahani2023dynamic,
bansak2024outcome, freund2024group}. The second approach focuses on designing a centralized \emph{preference-based} matching system that  respects the preferences of refugees and/or affiliates (see the work of \citet{nguyen2021stability} and \citet{delacretaz2023matching} and references therein). {While this approach has promise, most of the current programs, including the U.S. system, lack systematic data on preferences. Instead, they operate as a centralized outcome-based system.} 
%Although this approach is generally promising and in other contexts (e.g. helping asylum seekers) might be closer to practice, almost all current programs, including the U.S. system, do not explicitly elicit preferences from refugee families and instead operate as a centralized outcome-based system.
}
%\SLcomment{To discuss. Original version: ``While this approach has promise, most of the current programs, including the U.S. system, lack systematic data on preferences.''}
%\footnote{\revcolor{While discussing the rational behind this decision is beyond the scope of this paper, we believe it is connected to a combination of security-related reasons, as well as a belief that refugee preferences are not necessarily aligned with what is best for them in terms of getting resettled in the U.S.}}
% \RNdelete{There has been growing academic interest in designing matching policies for refugee resettlement, leading to the emergence of two main categories. The first category focuses on designing a centralized \emph{preference-based} matching system that can respect the preferences of refugees and/or affiliates (see, for example, the work of \citet{nguyen2021stability} and \citet{delacretaz2023matching} and references therein). Although this approach might be promosing in context such as , most of the current programs, including the U.S. system, lack systematic data on preferences. Instead, they operate as a centralized outcome-based system, focusing on integration outcomes such as employment within 90 days, given outcome predictions for various refugee profiles.} 



Several key factors distinguish our paper from past work: (i) {W}hile these work{s} focused on designing effective heuristics, we take a theoretical approach and propose algorithms with provable guarantees; %\footnote{We note that \citet{freund2024group} develops algorithms incorporating the notion of group fairness with a theoretical performance guarantee. However, this paper also assumes full knowledge of {the} arrival distribution.}
{(ii) {O}ur work focuses on operational and algorithmic intricacies due to post-allocation service and dynamics of backlogs, which have not been studied before;}
(iii) {T}he existing work designed algorithms that crucially rely on a pool of past years' data to either estimate the arrival distribution or simulate future arrivals. However, as elaborated in \Cref{subsec:intro+background}, such an approach can be \emph{non-robust} to discrepancies between the data from past years and the arrivals from the current year. In contrast, our algorithms are robust to such discrepancies, as they do not rely on data from previous years; and (iv) {A}s a result of such robustness, and in addition to enjoying theoretical guarantees, our method outperforms its counterpart in practical situations, as we discuss next.

{Among the existing work, \citet{bansak2024outcome} is the most appropriate point of comparison, since they also consider an objective that  penalizes congestion. However,  tied cases are not modeled, and thus the over-allocation cost is not included in the objective. %\RNedit{Moreover, they do not explicitly incorporate the specific dynamics of backlogs in the design of their algorithm, and provide no computationally efficient way of using this dynamic in their design.}
% \RN{I modified the last sentence a bit. Maybe Soonbong wants to take a pass based on what we discussed.}\EPcomment{I don't think the preceding sentence is accurate, since \citet{bansak2024outcome} has the same model/dynamics for backlog except for the stochastic server aspect.} 
We modify their proposed sampling-based algorithm to incorporate tied cases, %\RNedit{and to incorporate backlog dynamics in a computationally efficient way,} 
and then compare its performance with that of our method. As shown in  \Cref{sec:numerics}, our method performs substantially better due to its robustness.
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\bf Online Resource Allocation:}
{Online resource allocation problems have been extensively studied in operations and computer science. Given the broad scope of the literature, we only highlight the stream most closely related to our setting. For an overview of other streams of work in the literature, we refer the readers to \cite{mehta2007adwords} and \cite{huang2024online} for an informative survey.%\SLcomment{Footnote}\SLedit{(We also remark that our dynamic resources are also similar to the reusable resources studied in recent literature (see, for example, \cite{feng2022near} and references therein). However, the models in this stream of work do not allow for waiting for such resources.)}


As mentioned in \Cref{subsec:intro+contribution}, without dynamic resources, our setting reduces to the online resource allocation problem with an unknown i.i.d. arrival model. Several papers designed and analyzed algorithms for such settings. 
The primary intuition guiding the design is that, under the stochastic input model, we can \emph{learn} the arrival pattern by observing a small portion of the arrival data. Building on this intuition, earlier studies have explored primal methods~\citep{kesselheim2018primal} that periodically solve a linear program using the observed data, or dual-based methods that seek to efficiently learn the dual variables of the associated offline problem and avoid the computational costs associated with resolving. These methods work by one-time dual learning~\citep{devanur2009adwords, feldman2010online,molinaro2014geometry} (which is similar in nature to the ``predict-then-optimize'' approach, e.g., \cite{elmachtoub2022smart}), multiple-time dual learning~\citep{agrawal2014dynamic, li2022online}, or using adversarial online learning throughout the horizon~\citep{devanur2011near, agrawal2014fast, wang2014close, gupta2016experts, badanidiyuru2018bandits, balseiro2023best}. {All of these methods have also found further applications in various operational scenarios~\citep{chen2017revenue,zhalechian2022online}.}
%\SLcomment{To do for me Double check whether \cite{wang2014close} and \cite{agrawal2014fast} indeed belong to the right category}
%\SLcomment{\bf Question: is \citet{agrawal2014dynamic} related to adversarial online learning?}

Closest to our work is that of \citet{agrawal2014fast} and \citet{balseiro2023best}. These studies consider online resource allocation with an assumption that the (possibly convex) objective can only depend on {\em total} allocation of resources. Due to this assumption, the offline problem has only a few time-invariant dual variables, which can then be learned fast enough to ensure low regret. However, this assumption \emph{fails} for the average backlogs in our objective, where the associated dual variables are time-varying and thus cannot be learned using similar methods. This key difference led us to move beyond the techniques of the aforementioned papers, incorporating new tools from drift analysis and stochastic first-order methods to design and analyze low-regret algorithms. Specifically, our design and analysis of \CA{} (\Cref{ALG+Surrogate+D}) involve a novel combination of the drift-plus-penalty method \citep{neely2022stochastic} and adversarial online learning (see \Cref{subsec:ALG+D+pfsketch} and \Cref{apx:lyapunov}). Additionally, to analyze the drift of the backlog of \CO{}, we {utilize} a last-iterate high-probability convergence property of stochastic mirror descent, an unexplored direction in the literature on online resource allocation.
% \SLdelete{establish}

%Closest to our work is that of \citet{agrawal2014dynamic} and \citet{balseiro2021regularized} which also consider online resource allocation for an objective function that includes nonlinear convex terms. However, each of those terms can only be a function of {\em total} allocation of resources over the entire horizon. This condition is crucially leveraged in developing low-regret algorithms. In particular, thanks to this assumption, the offline problem has only a few time-invariant dual variables which can then be learned fast enough to ensure low regret. In our setting, the penalty terms for over-allocation satisfy this condition, and thus we use similar ideas to the aforementioned papers to learn their corresponding dual variables. However, such assumption {\em fails} for the average backlogs in our objective. The dual variables associated with these terms are time-varying and thus cannot be learned using similar ideas. This subtle difference led us to go well beyond the machinery of \citet{agrawal2014dynamic} and \citet{balseiro2021regularized} and to bring new tools from drift analysis and stochastic first-order methods (notably their last-iterate high probability convergence property we establish in \Cref{prop:harvey}) to design and analyze low-regret algorithms. 



%Rad: here is a longer version of the paragraph


% Another related line of work, started with the work of \cite{vera2019bayesian}, is the literature on minimizing regret for Bayesian online resource allocation~\citep{vera2021online,banerjee2020uniform,arlotto2020logarithmic,arlotto2019uniformly}. See \cite{balseiro2023survey} for a survey. Our work diverges from this line of work as the arrival distribution is assumed to be known in these models, and the main focus of the algorithms is to control the error propagation of decisions due to stochastic arrivals instead of learning the arrival. We also highlight that due to the backlog penalty term, our objective function does not satisfy the ``exchangeability'' condition imposed in the recent work of \cite{freund2019good}. This condition posits that the order and timing of actions do not impact the objective function's value. However, the backlog is inherently dynamic, and thus changing the order of arrivals or actions can significantly change the objective function.}

Another marginally related line of work is the literature on minimizing regret for Bayesian online resource allocation (see, for example, the work of  \cite{arlotto2019uniformly} and \cite{vera2019bayesian}). Our work diverges from this line of work as the arrival distribution is assumed to be known in these models, and the main focus of the algorithms is to control the error propagation of decisions due to stochastic arrivals instead of learning the arrival. Our dynamic resources are also similar to the reusable resources studied in recent literature (see, for example, \cite{feng2022near,gong2022online} and references therein). However, the models in this stream of work do not allow one to wait for such resources.} {As such, there is no notion of congestion or desire for a smooth matching.}

% We also highlight that due to the backlog penalty term, our objective function does not satisfy the ``exchangeability'' condition imposed in the recent work of \cite{freund2019good} in this. This condition posits that the order and timing of actions do not impact the objective function's value. However, the backlog is inherently dynamic, and thus changing the order of arrivals or actions can significantly change the objective function.}


%\SLcomment{Should we also highlight \cite{li2022online}? --- also studies convergence of the dual variables of the `resolving' methods (for reward maximization). They claim that their bound is high-probability, but I have not entirely understood their point. }

% dynamic resource: commented out. will use this if needed later 
%The dynamic resource in our study shares similarities with the \emph{reusable} resource, a topic actively explored in recent literature (see, for example, \cite{feng2022near} and references therein). Although the settings are incomparable in various aspects, there are notable differences. First, in our model, arrivals queue for the dynamic resource, introducing a queuing aspect not present in the cited papers. Secondly, we focus on an offline benchmark with complete knowledge of both arrivals \emph{and} resource availability. In contrast, the aforementioned papers focus on a clairvoyant online benchmark that only knows the arrival sequence, due to the impossibility of achieving a constant approximation for the full offline benchmark in the most general setting. Despite considering the offline benchmark, our algorithms achieve a sub-linear regret. Our result does not contradict the impossibility results established in the cited papers because (i) we consider a fundamentally different objective and constraints, and (ii) our impossibility result (\Cref{prop:impossibility}) also restricts any online algorithm from achieving sub-linear regret under specific parameter regimes.

\par 
{\bf Dynamic Matching and Control of Queueing Systems:} 
In queuing literature, a stream of work studies matching queues; in these systems, agents arrive over time and wait to be matched according to a deterministic compatibility structure \citep{aouad2020dynamic, aveklouris2021matching, afeche2022optimal, gupta2022greedy, hu2022dynamic, kerimov2023dynamic, wei2023constant} or a random one \citep{ashlagi2013kidney, anderson2017efficient, ashlagi2019matching}. While most of these papers focus on maximizing total (match-dependent) rewards, the work of \citet{aveklouris2021matching} considers an objective similar to ours that penalizes the matching reward by the cost of waiting. However, the crucial distinction of our paper from the aforementioned works is the {\em reverse order of matching and waiting}. As discussed in \Cref{subsec:intro+contribution}, our model can be viewed as a queuing system with an endogenous arrival rate controlled by the matching process. Once again, this subtle difference presents technical challenges in, for example, controlling the size of the backlog \revcolor{while performing learning and optimization.}
%Additionally, due to this difference, any online algorithm in our setting faces a fundamental limit in achieving sub-linear regret against our benchmark when the unit holding cost is too large (\Cref{prop:impossibility}).\VMcomment{Do we need to say this last sentence? I guess that \citep{aveklouris2021matching} can handle a large penalty factor but we cannot and tha't what you want to highlight?, but what's their benchmark? is this a fair comparison? Let's discuss! }\SLcomment{Let's remove this. }

From a methodological standpoint, the design and analysis of our first algorithm (\Cref{ALG+Surrogate+D}) partly rely on the celebrated drift-plus-penalty method \citep{tassiulas1990stability,lyapunov1992general,neely2006energy,neely2008fairness,neely2022stochastic} for stochastic network optimization and stability.  Our work complements this approach by combining the drift-plus-penalty method with adversarial online learning. Furthermore, our first algorithm implicitly utilizes the scaled backlog as a dual variable, establishing a crucial structural connection to the projected subgradient method \citep{zinkevich2003online}. A similar connection was observed in \cite{ashlagi2022price}  {and \cite{kanoria2023blind}}, albeit in a context different from the setup of our paper. We also note that, in a different context, \cite{wei2023constant} also integrates the drift-plus-penalty method with the resolving techniques.
%\ECcomment{To think of: should I cite ``Blind Dynamic Resource Allocation in Closed Networks via Mirror Backpressure"" by Yash Kanoria and Pengyu Qian?}\RNcomment{Yes!}\RNcomment{It would be great if we can make our further related work shorter and less defensive; I am happy to take a major pass and do it, if we feel that's how we want to write this.}\SLcomment{Done.}

==> tex/main/extensions.tex <==

{
\color{blue}
\section{Broader Applications}\label{subsec:broader+appl}
Our model can be applied to broader applications that share three key features: 
(i) real-time allocation of static resources with fixed capacity; 
(ii) each allocation triggers a time-consuming onboarding service from dynamic resources; and 
(iii) arrival patterns are not easily predicted from historical data gathered in prior planning horizons. In the following, we provide two examples of such applications. 
\smallskip 

\emph{(i) Hospital Operations.} 
Our model can support inpatient bed allocation decisions in hospitals. 
From a short-term planning perspective (e.g., daily or per-shift), each inpatient bed may be viewed as a static resource: admitting a patient consumes one unit of capacity for the remainder of the planning horizon. 
In addition, each admission triggers onboarding services — such as staff hand-off and patient transport — that require non-trivial time investments from hospital personnel (dynamic resources). 
These onboarding processes can delay treatment and are especially vulnerable to congestion when admissions occur in a bursty manner. 
For example, \citet{shi2016models} discusses post-(bed) allocation delays arising from shortages of nurses needed to coordinate patient transfers from the emergency department to inpatient wards. 
Finally, arrival patterns to hospitals often vary across planning horizons, and historical data may offer limited predictive value. For example,
day-to-day fluctuations in illness trends or local events could render past data unreliable for anticipating today’s arrival patterns.

Our framework captures the key trade-off in this setting: balancing the immediate benefit of allocating a bed (treating a patient) against the congestion of onboarding services. 
Our approach can support smooth  admission decisions that maximize treatment opportunities given limited bed capacity, while mitigating onboarding congestion. 
Furthermore, our learning-based approach makes such decisions robust to potentially unreliable historical data by taking a prior-free approach --- learning the current horizon’s arrival pattern in real time and adapting allocation decisions accordingly.\EPcomment{It isn't immediately obvious what the decision is in this context, since there may only be one department that each patient could go to (i.e., everyone is a tied case). Or, is the decision about \emph{when} to allocate someone to a bed? In this case, it is a bit different than the refugee context. Or are you only suggesting that the model is applicable, but not necessarily the algorithms?}



\smallskip 

\emph{(ii) Foster Care.} In 2021, more than 180{,}000 children entered the U.S. foster care system~\citep{acf_trends_2023}. While details vary across states, child welfare agencies are generally responsible for finding an initial foster placement shortly after a child enters the system. These early placements are intended to provide temporary stability—often lasting several days to a few weeks—until a permanent solution such as  adoption is pursued (for more institutional context, see \citet{robinsoncortes2021foster}). There has been growing academic interest in using data-driven approaches to improve foster care systems (see, for example, \citealt{slaugh2016pennsylvania} in the context of adoption matching).  

Our framework can support placement officers tasked with making these initial foster placement decisions. Within a reasonably short planning horizon—such as a month—each foster care facility (e.g., licensed foster homes or group care facility) can be viewed as a static resource with fixed capacity: once a child is placed, the corresponding slot is effectively occupied for the remaining horizon. In addition to consuming this static capacity, each placement triggers onboarding services such as follow-up monitoring by a case worker. Finally, the arrival patterns entering the system can fluctuate across planning horizons, making arrival patterns from the previous horizon an unreliable guide for the current one. For example, several counties have experienced a significant surge in foster care entries, driven in part by spikes in opioid misuse~\citep{radel2018substance}. Our model and learning-based algorithms can help placement officers find better matches between children and foster care facilities, while managing limited slots of the care facilities, avoiding overburdening onboarding service providers, and remaining robust to potentially unreliable historical data.}

==> tex/main/near+critical.tex <==
\begin{comment}
\subsection{Near-critical Regime}\label{sec:near+critical}
\end{comment}
% defnintion 

\Cref{thm:ALG+Surrogate+Primal} 
implies that \CO{} is equally powerful to \CA{} in the stable regime in the sense of achieving a sub-linear regret (even though it is oblivious to backlogs). However, through the following theorem, we show that \CO{} cannot achieve the same order of regret as \CA{} under the near-critical regime.

\begin{theorem}[Lower bound on Regret of \CO{} under Near-critical Regime]\label{thm:near+critical} There exists a constant $q>0$ and an instance such that for any given $\ServiceSlack \leq \frac{q}{\sqrt{\TotalTime}}$, the regret of $\CO{}$ is $\Omega(\gamma\sqrt{\TotalTime})$.
\end{theorem}

Together with \Cref{near+part+a} (see \Cref{subsec:ALG+D+pfsketch}), which states that the regret of \CA{} is $\BigO(\sqrt{\BuildUpCost\TotalTime})$ under the near-critical regime, \Cref{thm:near+critical} implies that \CA{} outperforms \CO{} with a better regret guarantee at least by a factor of $\sqrt{\BuildUpCost}$. In particular, \CO{} loses its ability to provide a sub-linear guarantee if $\BuildUpCost = \Theta(\TotalTime^{\delta})$ with $\delta \in [1/2, 1)$. Intuitively, such difference in the performance stems from the fact that \CA{} can adapt its behavior to the backlog by penalizing its scaled version with $\zeta = \Theta(\sqrt{\BuildUpCost/\TotalTime})$, whereas \CO{} cannot as it is oblivious to the backlog. Overall, this result highlights the inherent benefit of accounting for the backlog. 

%To establish this result, we revisit the one-location instance considered in Example \ref{example:stable} and conduct a delicate analysis of the algorithm's regret under the near-critical regime. Specifically, we demonstrate that the build-up at time $\Timeidx$ of the algorithm grows, in expectation, in the order of $\sqrt{\Timeidx}$ (this implies our desired $\Omega(\BuildUpCost \sqrt{\TotalTime})$ lower bound of regret). Interestingly, such `exploding' build-up arises from the algorithm 'targeting' the matching rate of $\boldsymbol{\CapRatio}$. To gain intuition, consider for a moment if the algorithm 'exactly' induces the matching rate of $\CapRatio$ at every period (similar to our analogy to the static policy introduced in Example \ref{example:stable}). In this case, due to the fact that $\ServiceSlack \leq O(1/\sqrt{\TotalTime})$, a simple anti-concentration result shows that, with constant probability, at least at time $\Timeidx$, there remains $\Omega(\sqrt{\Timeidx})$ build-up. As we elaborate in the proof, this intuition holds even when the algorithm's matching rate changes across time.


\begin{figure}[t]
  \centering
  \begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\linewidth]{images/fig+regret+ratio+final.png}
    \caption{$\textsf{Diff}^{\CO{}}/\textsf{Diff}^{\CA{}}$}
    \label{fig:critical+subfig1}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\linewidth]{images/fig+z_t+near+critical+final.png}
    \caption{$\E[\Decision_\Timeidx]$ for $\TotalTime=5000$ and $\ServiceSlack=0.5/\sqrt{\TotalTime}$}
    \label{fig:critical+subfig2}
  \end{subfigure}

  \caption{Numerical Illustrations for \Cref{thm:near+critical} with 1000 sample paths and $\boldsymbol{\BuildUpCost = \sqrt{\TotalTime}}$. We use notation $\boldsymbol{\textsf{Diff}^{\pi}}:= \boldsymbol{\E[\OPT(\BuildUpCost)] - \E[\textsf{ALG}^{\pi}(\BuildUpCost)]}$. The learning rate of \CA{} is $\boldsymbol{\eta = \frac{1}{\sqrt{\TotalTime}}}$, with $\boldsymbol{\zeta = \frac{10}{\sqrt{\TotalTime}}}$ ($\boldsymbol{\zeta = \sqrt{\frac{\BuildUpCost}{\TotalTime}}}$, resp.) under the stable regime (the near-critical regime, resp.). The learning rate of \CO{} is $\boldsymbol{\eta_\Timeidx = \frac{1}{\sqrt{\Timeidx}}}$ under both regimes. }
\end{figure}
%\SLdelete{, which was a one-location example consisting of only free cases whose the reward distribution is the uniform distribution on interval $(0,1)$. The capacity ratio is $\CapRatio=0.5$}

%to illustrate our analytic results through Figure \ref{fig:critical+subfig1}. Here we aim to describe (i) how the performance of the two algorithms differs in the near-critical regime and (ii) what leads to this difference in the performance.
In the proof of \Cref{thm:near+critical}, we revisit the \revcolor{single-affiliate} instance considered in Example \ref{example:stable} and conduct a delicate analysis of \CO{}'s regret under the near-critical regime. We defer the mathematical details of the proof to \Cref{apx+near+thm+proof}. 
\revcolor{Instead, in the following, we provide numerical evidence for the lower bound of regret in \Cref{thm:near+critical} by simulating our two algorithms under the same single-affiliate instance. In this numerical simulation,} for each $\TotalTime \in \{500,1000,...,5000\}$, we use $\BuildUpCost = \sqrt{\TotalTime}$ and $\ServiceSlack \in \{0.1, \frac{0.5}{\sqrt{\TotalTime}}, \frac{0.5}{{\TotalTime}}\}$, where the first value of $\ServiceSlack$ belongs to the stable regime and the other two to the near-critical regime. By using the notation of $\textsf{Diff}^{\pi} := \E[\OPT(\BuildUpCost)] - \E[\textsf{ALG}^{\pi{}}(\BuildUpCost)]$ for an algorithm $\pi$ {(note that $\OverCost$ does not play any role in this instance because there are no tied cases)}, 
%\footnote{\SLedit{Because there are no tied cases in this instance, $\OverCost$ does not play any role. Hence, we omit its dependence.}} 
we display $\textsf{Diff}^{\CO{}}/\textsf{Diff}^{\CA{}}$ in Figure \ref{fig:critical+subfig1} (as a function of $\TotalTime$).  
%\VMcomment{no $\alpha$ b/c there is no tied cases?}\SLcomment{yes, mentioned in the footnote}
Consistent with \Cref{thm:near+critical} and \Cref{near+part+a}, we note that the ratios (two red curves) diverge in the order of $\sqrt{\BuildUpCost} = \TotalTime^{1/4}$ under the near-critical regimes. In contrast, the ratio under the stable regime (blue curve) remains constant, which is also consistent with Theorems~\ref{thm:ALG+Surrogate+Dual} and \ref{thm:ALG+Surrogate+Primal}. However, we observe that \CA{} still achieves a lower regret than \CO{} by a constant factor (roughly 70\%). \par 

The main reason behind the performance difference lies in the endogenous arrival rates that each algorithm's decision induces. More specifically, Figure \ref{fig:critical+subfig2} illustrates the empirical average of $\Decision_\Timeidx$ (solid line) for $\TotalTime=5000$ and $\ServiceSlack = 0.5/\sqrt{\TotalTime}$, which serves as a proxy for the (expected) endogenous arrival rates. The arrival rate of \CO{} quickly converges to $\CapRatio=0.5$, as evident from the cumulative time-average (dashed red line). In contrast, \CA{} induces an arrival rate strictly less than $\CapRatio=0.5$ (dashed blue line). Under the stable regime, maintaining an induced arrival rate of $\CapRatio$ ensures a constant average backlog. However, in the near-critical regime, we can show that the approach of \CO{} results in a time-average backlog of $\Omega(\TotalTime^{1/2})$ for this specific instance (see \Cref{lemma:all+time+build}). To gain some intuition, consider momentarily that the algorithm ``exactly'' induces the matching rate of $\CapRatio$ at every period. Because $\ServiceSlack=\BigO(1/\sqrt{\TotalTime})$, a simple anti-concentration result implies that, with constant probability, there remains $\Omega(\sqrt{\Timeidx})$ \backlog{} at each period $\Timeidx$. By contrast, by penalizing the current backlog level, \CA{} achieves a better order of the backlog (and thus, a better order of regret).%\SLcomment{Main body up to this point:}

%In contrast, \CA{} effectively targets an arrival rate strictly less than $\CapRatio=0.5$, leading to a better order of \backlog{} (and therefore a better regret) while maintaining a sub-linear loss of the reward. 

\begin{comment}
We summarize our analytic results by using \Cref{fig:regret+ratio}. In the figure, we draw the ratio of the regret of \Cref{ALG+Surrogate+P} to that of \CA{} as a function of $\TotalTime$ under $\BuildUpCost =\sqrt{\TotalTime}$. We consider three different regimes regarding $\ServiceSlack$. For each regime, we consider an instance of one location ($m=1$) and the capacity ratio of $\rho=0.5$, and every arrival is a free case. The blue curve shows the regret ratio under the stable regime with $\ServiceSlack=0.1$. The reward under this regime is drawn from Uniform[0,1] distribution, which satisfies Assumptions \ref{ass:conti} and \ref{assump:M}. The two red curves consider the near-critical regime, each with $\ServiceSlack = \frac{0.5}{\sqrt{\TotalTime}}$ and $\ServiceSlack = \frac{0.5}{\TotalTime}$, respectively, as a function of $\TotalTime$. We use the reward distribution studied in the proof of \Cref{thm:near+critical}-(b) where \Cref{ALG+Surrogate+P} provably faces a barrier of $\Omega(\BuildUpCost\sqrt{\TotalTime})$ regret. The step size of \Cref{ALG+Surrogate+D} is $\eta=\frac{1}{\sqrt{\TotalTime}}$, $\zeta = \frac{10}{\sqrt{\TotalTime}}$ under the stable regime and $\zeta = \sqrt{\frac{\BuildUpCost}{\TotalTime}}$ under the near-critical regime. The step size of \Cref{ALG+Surrogate+P} is $\eta_\Timeidx = \frac{1}{\sqrt{\Timeidx}}$ under both regimes. \par 
Focus on the red curves corresponding to the near-critical regime, we note that the regret ratios in both red curves diverge in the order of $\sqrt{\BuildUpCost} = \TotalTime^{1/4}$, while the magnitude of the ratio increases by a constant factor as $\ServiceSlack$ shrinks. In contrast, the regret ratio under the stable regime (blud curve) remains constant. Said differently, the two algorithm achieve the same order of regret in $\TotalTime$. However, somewhat interestingly, we observe that \Cref{ALG+Surrogate+D} still achieves a lower regret than \Cref{ALG+Surrogate+P} by a constant factor (roughly by 70\%).\SLcomment{What would be a good sentence to wrap up this paragraph?}. \par 
\end{comment}

\begin{comment}
We conclude this section by highlighting the main difference between \Cref{ALG+Surrogate+D} and \Cref{ALG+Surrogate+P} on the instance studied for the proof of \Cref{thm:near+critical}-(b). We have shown that \Cref{ALG+Surrogate+P} faces $\Omega(\BuildUpCost\sqrt{\TotalTime})$ because its average build-up is $\Omega(\sqrt{\TotalTime})$ for any value of $\BuildUpCost$. Said differently, the fact that \Cref{ALG+Surrogate+P} completely ignores the presence of the build-up hurts the algorithm in the near-critical regime. In contrast, $\Cref{ALG+Surrogate+D}$ \par

We have shown that the average build-up of \Cref{ALG+Surrogate+P} is $\Omega(\sqrt{\TotalTime})$ in expectation in the near-critical regime. Notably, the result holds for \emph{any} values of $\BuildUpCost$ because the decision of \Cref{ALG+Surrogate+D} does not depend on $\BuildUpCost$. 

In contrast, \Cref{ALG+Surrogate+D} is able to obtain a better guarantee on the build-up by $\O(\sqrt{\TotalTime/\BuildUpCost})$ by setting $\zeta = \Theta(\sqrt{\TotalTime/\BuildUpCost})$ as a function of $\BuildUpCost$ while also incurring an additional loss of reward. Said differently, 
    
\end{comment}


==> tex/main/related+lit.tex <==
Our work relates to and contributes to several streams of literature.\par 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\SLcomment{This section needs a complete overhaul: (1) make it shorter and direct, especially by focusing on dynamic refugee matching (2) push the preference-based matching to last.}
{\bf Matching Policies for Refugee Resettlement:} There has been growing academic interest in designing matching policies for refugee resettlement, leading to the emergence of two main categories. The first category, primarily developed in economics, focuses on designing a centralized \emph{preference-based} matching system \citep{andersson2018dynamic, delacretaz2019matching, jones2017international, jones2018local, nguyen2021stability}. Leveraging the theory of mechanism design, these papers focus on developing a matching policy with desirable properties related to the preferences of refugees and/or affiliates.

The second category, to which our paper also belongs, involves the development of \emph{outcome-based} matching policies.  
This approach is motivated by the availability of historical administrative data on refugees that contains information on their initial placement and integration outcomes (e.g., 90-day employment outcome), along with demographic characteristics. These datasets enable the training of a supervised learning algorithm predicting employment outcomes in each affiliate based on refugee demographics. \cite{bansak2018improving} pioneered this approach in studying the geographic assignment of refugees under the capacity constraints of each location affiliate. \cite{ahani2021placement} extended the same approach with more extensive constraints, and \cite{golz2019migration} complemented previous works by incorporating the competition effect, where refugees assigned to the same affiliate compete for jobs with limited availability. However, all these works exclusively consider the static assignment of refugees. In practice, refugees arrive sequentially, and therefore, our work focuses on the \emph{dynamic} (sequential) resettlement of refugees.

Several recent works have studied the dynamic assignment of refugees \citep{ahani2021dynamic, bansak2022outcome, freund2024group}. The first paper focuses on maximizing the total employment outcome, while the last two additionally consider allocation balancing across time and group fairness, respectively. We diverge from these papers in two aspects. Firstly, the preceding works do not consider the impact of tied cases. We formally incorporate this factor and the resulting cost of over-allocation into our objective. Secondly, existing proposals require knowledge of the arrival distribution or access to a sample trajectory of future arrivals from a sampling pool, which consists of data from previous years. However, relying heavily on such prior information can render these algorithms \emph{non-robust} to potential discrepancies between the sampling pool and the current year's arrivals. Indeed, as shown in Figure \ref{fig:tied+proportion}, the proportion of tied cases in the real data from our partner agency exemplifies such discrepancies. Motivated by this observation, we aim to develop a \emph{prior-robust} algorithm that requires no prior knowledge of the arrival distribution (except the assumption of stationarity when provng the theoretical guarantees). In Section \ref{sec:numerics}, we further illustrate the robustness of our algorithm in real-world, non-stationary settings, and show that this increased robustness translates into substantial improvements relative to benchmark methods. %\EPcomment{I am trying to disentangle the need for stationarity in the theoretical results versus the fact that we don't need stationarity in order for the algorithm to work well in practice}\SLcomment{incorporated}

%% WORKED SO FAR HERE %%%% 
Finally, our paper shares similarities with \cite{bansak2022outcome} regarding the use of a queuing system to define the measure of allocation balance across time. However, crucial differences exist: (i) we allow for a stochastic service with arbitrary service slack (see \Cref{sec:model}), whereas \cite{bansak2022outcome} only permits a fully deterministic service flow with no service slack; (ii) the aforementioned work adopts a simulation-based approach to evaluate the algorithm's performance, while we take a theoretical perspective and offer a formal analytic guarantee of performance, enhancing its generalizability beyond a specific set of simulation results.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\bf Online Resource Allocation:}
Online resource allocation problems have been extensively studied in operations research. Given the broad scope of the literature, we only highlight recent advances and kindly refer readers to \cite{mehta2007adwords} and \cite{balseiro2023survey} for an informative survey.

A classical setup of this problem involves allocating an endowed amount of static (i.e., non-reusable) resources to sequentially arriving agents, who then consume a certain amount of the resource, to maximize the total matching reward collected. The primary framework for evaluating performance is to compare the performance of an online algorithm to that of the \emph{hindsight} optimal solution (also known as the offline solution) with full knowledge of arrival sequences upfront. It is well-known that under the fully adversarial arrival model, no online algorithm can obtain a constant-factor approximation of the hindsight optimum \citep{aggarwal2011online} for the general online allocation problem. To overcome this impossibility, the literature has focused on the (stationary) \emph{stochastic} arrival model where the arrival is drawn from a (potentially unknown) distribution, either with (known as the \emph{i.i.d. model}) or without replacement (known as the \emph{random permutation model}). Our work also assumes the i.i.d arrival model and therefore is broadly connected to the stream of the stochastic input model. In particular, we focus on designing a \emph{prior-robust} algorithm that can perform well across all stationary arrival distributions \emph{without} knowing them.\footnote{For \emph{prior-dependent} algorithms with knowledge of the arrival distribution, we kindly refer reader to \cite{balseiro2023best} and references therein for an informative survey.}

% Distribution-free online algs 1: first generation (periodic resolving)
The primary intuition guiding the design of a prior-robust online algorithm is that, under the stochastic input model, we can \emph{learn} the arrival pattern by observing a small portion of the arrival data. Building on this intuition, earlier studies have explored dual-based \citep{devanur2009adwords, feldman2010online, agrawal2014dynamic, li2022online} or primal-based \citep{kesselheim2018primal} methods that periodically solve a linear program using the observed data. 

Recognizing the computational costs associated with these algorithms, the recent stream of works, which our paper also belongs to, has further focused on an efficient algorithm that circumvents the need for solving the auxiliary optimization program. The relevant papers in this stream include \cite{devanur2011near, agrawal2014dynamic, gupta2016experts, balseiro2023best}, and \cite{balseiro2021regularized}. These papers leverage \emph{online learning} (also known as online convex optimization) problem to efficiently update dual variables that guide resource allocation. The papers most closely related to ours are \cite{balseiro2023best} and \cite{balseiro2021regularized}. The former proposes the dual-mirror descent method to maximize total reward under the hard resource constraint of static resources. The latter extends a similar algorithm to incorporate a convex regularizer as a function of the \emph{total} resource consumption. In our approach, we adopt a similar strategy of employing the mirror-descent method for updating dual variables. Consequently, our algorithm yields a similar updating rule of the dual variables (for the static resource) as the aforementioned papers. 

We highlight three main differences from the literature on online learning-based algorithms. Firstly, our objective function introduces the cost of average backlogs for the dynamic resource, which in general cannot be expressed as a convex function of the total resource consumption \SLedit{even when the service rate equals to the capacity ratio}. Secondly, due to the presence of the dynamic resource, our proposed algorithms require significantly different proof techniques. For the first algorithm (see \Cref{ALG+Surrogate+D}), which has access to the congestion level of the dynamic resource, we successfully integrate drift analysis \citep{neely2022stochastic} and the adversarial regret guarantee of online mirror descent.  Furthermore, we establish a novel connection for our second algorithm (\Cref{ALG+Surrogate+P}), which is agnostic to the dynamic resource, to the last iterate convergence of the \emph{stochastic} mirror descent \citep{harvey2019tight}. We leverage this connection to demonstrate that, under specific regimes, our second algorithm achieves remarkably low congestion levels in the dynamic resource. This finding is the first of its kind in the literature, to the best of our knowledge. Finally, we illustrate the failure of the second algorithm under certain regimes, underscoring the necessity for a new algorithm accounting for the dynamic resource.
\SLcomment{Worth mentioning more if space permits: \cite{li2022online} --- also stuies convergence of the dual variables of the `resolving' methods. }

% dynamic resource
The dynamic resource in our study shares similarities with the \emph{reusable} resource, a topic actively explored in recent literature (see, for example, \cite{feng2022near} and references therein). Although the settings are incomparable in various aspects, there are notable differences. First, in our model, arrivals queue for the dynamic resource, introducing a queuing aspect not present in the cited papers. Secondly, we focus on an offline benchmark with complete knowledge of both arrivals \emph{and} resource availability. In contrast, the aforementioned papers focus on a clairvoyant online benchmark that only knows the arrival sequence, due to the impossibility of achieving a constant approximation for the full offline benchmark in the most general setting. Despite considering the offline benchmark, our algorithms achieve a sub-linear regret. Our result does not contradict the impossibility results established in the cited papers because (i) we consider a fundamentally different objective and constraints, and (ii) our impossibility result (\Cref{prop:impossibility}) also restricts any online algorithm from achieving sub-linear regret under specific parameter regimes.

\par 
{\bf Dynamic Matching and Control of Queueing Systems:} In the model of dynamic matching of queues, each type of agent arrives and waits in the queue until it is matched with agents of other types, either in a bipartite \citep{aveklouris2021matching, afeche2022optimal} or multiway \citep{kerimov2023dynamic, gupta2022greedy, wei2023constant} manner. Our modeling of the arrivals joining the queue for the dynamic resource bears resemblance to the models of dynamic matching in queueing systems. Closer to our work is \cite{aveklouris2021matching}. This paper focuses on maximizing total (match-dependent) rewards minus the holding costs of agents in the queue. We also consider a similar objective function including the time-average queue length for the dynamic resource. The crucial distinction in our paper from the aforementioned works lies in the timing of waiting. The models in the aforementioned papers follow a \emph{wait-then-match} framework: the agent joins the queue and then waits until the match is performed. In contrast, our setting is based on a \emph{match-then-wait} framework: the match is first performed, and then the agent joins the queue at the matched location for \emph{post-allocation} services. Due to this difference, any online algorithm in our setting faces a fundamental limit in achieving sub-linear regret against our benchmark when the unit holding cost is too large (\Cref{prop:impossibility}).\par 
From a methodological standpoint, the design and analysis of our first algorithm (\Cref{ALG+Surrogate+D}) in part builds on the drift-plus-penalty method \citep{ neely2022stochastic} for stochastic network optimization. We remark that \cite{wei2023constant} also integrates the drift-plus-penalty method with the resolving technique to account for estimation errors of the dual variables. Our work complements this approach by combining the drift-plus-penalty method with the online learning method. Additionally, our first algorithm implicitly utilizes the scaled queue length as a dual variable, establishing a profound structural connection to the projected subgradient method \citep{zinkevich2003online}. A similar connection was observed in \cite{ashlagi2022price}, albeit in a different context from the setup of our paper.
\begin{comment}
Our paper is related to the literature on dynamic resource allocation and refugee matching. In this section, we provide a brief review of the relevant papers and how this paper contributes to each stream of work. \par 
\textbf{Design and Analysis of Refugee Matching Policy:} There has been emerging academic interest in designing a matching policy for refugee resettlement. Within this stream, two main categories have developed. The first category, developed primarily in economics, aims to build a centralized \emph{preference-based} matching system. The papers in the this category \citep{andersson2018dynamic, delacretaz2019matching, jones2017international, jones2018local, nguyen2021stability} are mainly motivated by the economic theory of the matching mechanism. These papers have studied theoretical matching policies with desirable properties related to the preference of refugees and (or) affiliates. \par 
The second category, found primarily in operations research, develops \emph{outcome-based} matching policies based on optimization algorithms. 
Our paper is more related to this category. The outcome-based optimization approach is motivated by the availability of data that records historical resettlement results of refugees (e.g., their initial placement and the 90-day employment outcome) as well as the refugee's demographic characteristics. Such data sets enable us to train a supervised learning algorithm that predicts the employment outcome in each affiliate as a function of the refugee's demographic characteristics. \cite{bansak2018improving} was the first to take this approach to study a \emph{static} assignment of refugees. They use the predicted employment outcome as input into the integer programming to find an optimal assignment that maximizes the total employment outcome subject to the capacity constraints of each affiliate. \cite{ahani2021placement} extended the same approach with some expanded resource constraints.   \cite{golz2019migration} complemented the previous work by incorporating the competition effect in which refugees assigned to the same affiliate would compete for jobs with limited availability. However, all of these works only consider the static assignment of refugees. As discussed in Section \ref{background}, refugees arrive sequentially at each voluntary agency. \par 
Our work focuses on the \emph{dynamic} refugee assignment. Few recent works have studied the dynamic assignment of refugees \citep{ahani2021dynamic, bansak2022outcome}, and these two works are closest to ours. Both papers model the dynamic refugee assignment as a special instance of the online generalized assignment problem. The algorithms proposed in both papers sample future arrivals from historical data (e.g. data from past years) to solve many instances of an offline matching problem. The difference between the two papers is that while \cite{bansak2022outcome} use the \emph{primal} solutions of the offline matching, \cite{ahani2021dynamic} use the \emph{dual} variables to guide the primal decision. However, we highlight two differences from the preceding works. First, the proposed algorithms are \emph{agnostic} to the arrival of tied cases. Our paper is the first to formally incorporate the tied cases and the resulting risk of over-allocation. Hence, we provide a more complete and general modeling framework. Secondly, the existing proposals all require access to a sample trajectory of future arrivals based on the sampling pool of data from previous years. However, the heavy reliance on historical data can make these algorithms \emph{non-robust} to any potential discrepancy between the sampling pool and the current year's arrival. For example, as we have highlighted Figure \ref{fig:tied+proportion}, the composition of free and tied cases varies significantly across different years. Relying on the projection of the tied cases based on the historical data can significantly mislead the algorithm. In contrast, rather than relying on the sampling process of future arrivals, our proposed algorithm \emph{learn} the arrival pattern in real time as we make the allocation decision. Lastly, the preceding works take a simulation-based approach to justify the performance. In contrast, we take a theoretical perspective and provide a formal analytic guarantee of the performance, making it much more generalizable beyond a set of simulation results. \par
% 
\textbf{Dynamic allocation of static resources:} Online resource allocation problems have been extensively studied in operations research and computer science literature. In this problem, the main focus is to design a policy that allocates static (offline) resources to sequentially arriving requests. Given the scope of the rich literature, we focus only on papers most relevant to our project. For a more in-depth review, we kindly refer the reader to \cite{mehta2013online} and \cite{balseiro2022best}. \par 
The main problem in this literature is to efficiently allocate (i.e. match) the initially endowed \emph{static} resources (often called \emph{offline} resources) to sequentially arrive at online requests to maximize the matching outcome. The main framework of performance evaluation is to compare the performance of an online algorithm to that of the \emph{hind-sight} optimal policy which knows the arrival sequence upfront. It is well known that under the fully adversarial arrival model, no online algorithm can obtain a constant-factor approximation of the hindsight optimum \citep{aggarwal2011online} for the online generalized assignment problem. To avoid this impossibility, To avoid this impossibility result, previous work has focused on two directions. The first direction is to impose a special structure on the problem, such as the consumption of resources proportional to the rewards \citep{mehta2007adwords, buchbinder2007online, golrezaei2014real} or the free disposal of the online nodes \citep{feldman2009online, devanur2016whole}. The second direction, which our paper also belongs to, is to consider \emph{stochastic} arrival models such as the random permutation model or the IID model with unknown distribution. In the random permutation model, there is a sequence of inputs fixed in advance but unknown to the algorithm, and these arrivals come in a uniformly random order. In the unknown IID distribution model, an arrival input at each time is an IID sample from an unknown distribution.  \par 
Several algorithms have been developed for the stochastic arrival models and have been shown to attain the near-optimal performance guarantee. One of the well-studied algorithms is a primal-dual algorithm, which utilizes a dual solution of the offline program to price the resource and use an opportunity-cost adjusted reward to guide the primal decision.  The key in the primal-dual algorithm is how to learn the good dual variables that can provide good primal performance. The initial approach in this stream was to solve a dual program after observing a portion of arrivals and use the dual solution as a shadow price. This approach was first studied by \cite{devanur2009adwords} in the Adwords problem under the random permutation model. \cite{feldman2010online} studied a similar algorithmic principle in Display Ad Allocation with the unknown IID distribution model. Both papers solve the dual programming \emph{once} with some fraction of arrivals. \cite{agrawal2014dynamic} further improved this technique with better performance by solving the dual program multiple times with carefully chosen time steps. \par 
The closest papers on the primal-dual algorithm to ours are \cite{agrawal2014fast} and \cite{balseiro2022best, balseiro2021regularized}. These papers propose a primal-dual algorithm that updates the dual variable using a black-box online learning algorithm. The seminal work of \cite{agrawal2014fast} initiated this line of work. The framework can be applied to any optimization with a general convex function defined on the \emph{aggregate} consumption of the static resources. We also use a similar idea to deal with the regularizer for the over-allocation. The algorithm proposed in this work requires an estimate of the value of the hindsight optimum or needs to solve an auxiliary optimization program to obtain an estimate of it. \cite{balseiro2022best} further extends this methodology by proposing a similar algorithm that does not require solving any auxiliary program. Recently, \cite{balseiro2021regularized} also extended their algorithmic idea to a setting with a fairness regularizer on the aggregate consumption of the static resources. \par 
Our paper contributes to this line by incorporating an objective function regarding the congestion of \emph{dyanamic resources}. We
properly define a queue for each dynamic resource and add the average queue size as a regularizer, which cannot be expressed as a function of \emph{aggregate} consumption of the static resources. A sequential structure of the queue size induces a high-dimensional set of corresponding dual variables. However, by observing the connection between the projected gradient descent and the queue size, we successfully incorporate the idea of the online learning method to design a policy that can balance the queue size with little loss of the total rewards. \par  \par 

\textbf{Dynamic matching in queueing systems:} In a broad sense, our paper is also related to the literature on matching and control of queueing systems, either bipartite \citep{aveklouris2021matching, afeche2022optimal} or multiway \citep{kerimov2023dynamic, gupta2022greedy, wei2023constant}. Our work significantly differs from this stream work in two ways. First, the timing of waiting is different. In the literature on queueing systems, the agents wait \emph{before} the matching decision is executed. However, in our setting, the agents wait \emph{after} the matching decision is executed. Second, these stream works do not consider a capacity constraint on the static resources. In fact, these crucial difference prevents any online algorithm from achieving a near-optimal performance guarantee when the cost for queue size is to large (Proposition \ref{prop:impossibility}).\par 
On the technical side, the analysis of our algorithm is inspired by the drift-plus-penalty method \citep{hwang2021online} for controlling a stochastic network. We successfully combine the technique with the online learning method to prove a regret guarantee in the presence of \emph{both} dynamic and static resources. A key observation of proving our main result is a connection between the well-celebrated projected subgradient descent \citep{zinkevich2003online} and the evolution of the queue size. Similar connections have been noted and used for analysis in \cite{huang2009delay} and \cite{ashlagi2022price}, although they focus on the infinite-horizon system and the steady-state performance in the long run. In contrast, we focus on a regret performance on the finite horizon. 
% + need to mention sophie's paper as they also use this interpretation (drfit-plus-penalty).    
\end{comment}

